Robust Symmetry Detection via Riemannian Langevin Dynamics

Symmetries are ubiquitous across all kinds of objects, whether in nature or in man-made creations. While these symmetries may seem intuitive to the human eye, detecting them with a machine is nontrivial due to the vast search space. Classical geometry-based methods work by aggregating "votes" for each symmetry but struggle with noise. In contrast, learning-based methods may be more robust to noise, but often overlook partial symmetries due to the scarcity of annotated data. In this work, we address this challenge by proposing a novel symmetry detection method that marries classical symmetry detection techniques with recent advances in generative modeling. Specifically, we apply Langevin dynamics to a redefined symmetry space to enhance robustness against noise. We provide empirical results on a variety of shapes that suggest our method is not only robust to noise, but can also identify both partial and global symmetries. Moreover, we demonstrate the utility of our detected symmetries in various downstream tasks, such as compression and symmetrization of noisy shapes.

==> figures/mode_seeking.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{images/onecol.pdf}
\caption{
    \textbf{A demonstrative figure for the mode seeking process with math notations?}.
    }
\label{fig:mode_seeking}
\end{figure}

==> figures/sparse.tex <==
\begin{figure*}[ht]
\centering
    \hspace{1cm} 4 views \hspace{5.6cm} 6 views \hspace{5.6cm} 8 views\\
    \includegraphics[width=\linewidth]{images/sparse_comp.pdf}
    \vspace{-2em}
    \caption{Applications in symmetry fixing for noisy shapes. We show fixed shapes based on the detected symmetry planes on a generated noisy shape. 
     }
    \label{fig:sparse}
    \vspace{-1em}
\end{figure*}


==> sections/ablations.tex <==
\section{Ablation study}
\label{sec:ablations}
With hyperparameter tuning, we achieve the best performance with: kernel size = 0.025, $k$ = 0.3, step size = 0.06 for 2D, and kernel size = 0.08, $k$ = 0.5, step size = 0.02 for 3D. We use 200 points for Langevin initialization and take 50K steps for both. We show the effects of altering such parameters in the results section.

%\input{tables/hyperparams}
%\input{tables/dbscan_ablate}
